Map-based cosmology inference with weak lensing -- information content and its dependence on the parameter space

Field-level inference is emerging as a promising technique for optimally extracting information from cosmological datasets. Indeed, previous analyses have shown field-based inference produces tighter parameter constraints than power spectrum analyses. However, estimates of the detailed quantitative gain in constraining power differ. Here, we demonstrate the gain in constraining power depends on the parameter space being constrained. As a specific example, we find that field-based analysis of an LSST Y1-like mock data set only marginally improves constraints relative to a 2-point function analysis in $\Lambda$CDM, yet it more than doubles the constraining power of the data in the context of $w$CDM models. This effect reconciles some, but not all, of the discrepant results found in the literature. Our results demonstrate the importance of using a full systematics model when quantifying the information gain for realistic field-level analyses of future data sets.

==> sections/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

Related papers:
\begin{itemize}
    \item \citep{Porth2021}: Tested the information content of 2D projected fields with Quijote simulations. Find $\sim 5$ times improvement in constraining power at $4~h^{-1}$ Mpc. 
    \item \citep{Porqueres2022}: Find a big improvement with BORG-WL at intermediate resolution. Likely wrong power spectrum results.
    \item \citep{Dai2022}: Normalizing flow based priors. Find $\gtrsim 5$ times improvement in constraining power at $4~h^{-1}$ Mpc. 
    \item \citep{Ribli2019}: CNN based analysis for weak lensing. Finds 2-3 times more information at ~1 arcminute resolution.  
    \item \citep{Cheng2020}: Scattering transforms based analysis for weak lensing. Agreement with CNN.
    \item \citep{Grewal2022}: Minkowski functionals for both convergence fields and galaxy density fields
    \item \citep{Ajani2022}: Starlet with galaxy clustering data non-Gaussianity.
    \item ..........
\end{itemize}
